Data Poisoning Attacks Against Federated Learning Systems

Federated learning (FL) is an emerging paradigm for distributed training of large-scale deep neural networks in which participants' data remains on their own devices with only model updates being shared with a central server. However, the distributed nature of FL gives rise to new threats caused by potentially malicious participants. In this paper, we study targeted data poisoning attacks against FL systems in which a malicious subset of the participants aim to poison the global model by sending model updates derived from mislabeled data. We first demonstrate that such data poisoning attacks can cause substantial drops in classification accuracy and recall, even with a small percentage of malicious participants. We additionally show that the attacks can be targeted, i.e., they have a large negative impact only on classes that are under attack. We also study attack longevity in early/late round training, the impact of malicious participant availability, and the relationships between the two. Finally, we propose a defense strategy that can help identify malicious participants in FL to circumvent poisoning attacks, and demonstrate its effectiveness.

==> results/1B-table.tex <==
\begin{table}[ht]
    \vspace{-6pt}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{|ccc|c|c|c|c|c|c|c|c|}
        \hline
        \multirow{2}{*}{\shortstack{$c_{src}$}} & \multirow{2}{*}{$\rightarrow$} & \multirow{2}{*}{\shortstack{$c_{target}$}} & \multirow{2}{*}{\shortstack{$m\_cnt^{src}_{target}$}} & \multicolumn{7}{c|}{Percentage of Malicious Participants ($m\%$)} \\
        \cline{5-11}
        & & & & 2 & 4 & 10 & 20 & 30 & 40 & 50 \\
        \hline
        \multicolumn{11}{|c|}{CIFAR-10} \\
        \hline
        0 & $\rightarrow$ & 2 & 16 & \cellcolor{yellow}{\textbf{1.42\%}} & 2.93\% & \cellcolor{yellow}{\textbf{10.2\%}} & 14.1\% & 48.3\% & \cellcolor{yellow}{\textbf{73\%}} & \cellcolor{yellow}{\textbf{70.5\%}} \\
        % \hdashline
        1 & $\rightarrow$ & 9 & 56 & 0.69\% & \cellcolor{yellow}{\textbf{3.75\%}} & 6.04\% & 15\% & 36.3\% & 49.2\% & 54.7\% \\
        % \hdashline
        5 & $\rightarrow$ & 3 & 200 & 0\% & 3.21\% & 7.92\% & \cellcolor{yellow}{\textbf{25.4\%}} & \cellcolor{yellow}{\textbf{49.5\%}} & 69.2\% & 69.2\% \\
        \hline
        \multicolumn{11}{|c|}{Fashion-MNIST} \\
        \hline
        1 & $\rightarrow$ & 3 & 18 & 0.12\% & 0.42\% & 2.27\% & 2.41\% & \cellcolor{yellow}{\textbf{40.3\%}} & \cellcolor{yellow}{\textbf{45.4\%}} & 42\% \\
        4 & $\rightarrow$ & 6 & 51 & \cellcolor{yellow}{\textbf{0.61\%}} & \cellcolor{yellow}{\textbf{7.16\%}} & \cellcolor{yellow}{\textbf{16\%}} & \cellcolor{yellow}{\textbf{29.2\%}} & 28.7\% & 37.1\% & \cellcolor{yellow}{\textbf{58.9\%}} \\
        6 & $\rightarrow$ & 0 & 118 & -1\% & 2.19\% & 7.34\% & 9.81\% & 19.9\% & 39\% & 43.4\% \\
        \hline
    \end{tabular}
    }
    \caption{Loss in source class recall for three source $\rightarrow$ target class settings with differing baseline misclassification counts in CIFAR-10 and Fashion-MNIST. Results are averaged from 10 runs. Highlighted bold entries indicate highest loss in source class recall in each setting.} %% Results are averaged from 10 runs for each setting of $m\%$ and source, target classes for both datasets.
    \label{tab:1B}
    \vspace{-34pt}
\end{table}
